ManiFlow: Implicitly Representing Manifolds with Normalizing Flows

Normalizing Flows (NFs) are flexible explicit generative models that have been shown to accurately model complex real-world data distributions. However, their invertibility constraint imposes limitations on data distributions that reside on lower dimensional manifolds embedded in higher dimensional space. Practically, this shortcoming is often bypassed by adding noise to the data which impacts the quality of the generated samples. In contrast to prior work, we approach this problem by generating samples from the original data distribution given full knowledge about the perturbed distribution and the noise model. To this end, we establish that NFs trained on perturbed data implicitly represent the manifold in regions of maximum likelihood. Then, we propose an optimization objective that recovers the most likely point on the manifold given a sample from the perturbed distribution. Finally, we focus on 3D point clouds for which we utilize the explicit nature of NFs, i.e. surface normals extracted from the gradient of the log-likelihood and the log-likelihood itself, to apply Poisson surface reconstruction to refine generated point sets.

==> figs/architectures/architectures.tex <==
\begin{figure*}
\centering
\begin{subfigure}{.9\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figs/architectures/softflow.pdf}
  \caption{Basic module of architecture used in comparison with SoftFlow~\cite{kim2020softflow}.}.
  \label{fig:softflow_architecture}
\end{subfigure}%
\\
\begin{subfigure}{.9\textwidth}
  \centering
  \includegraphics[width=.9\linewidth]{figs/architectures/dpf.pdf}
  \caption{Basic module of RealNVP architecture used in general comparison on point cloud autoencoding.}
  \label{fig:dpf_architecture}
\end{subfigure}
\caption{Architectures used in comparison in \secref{subsubsection:softflow} (a) and \secref{subsection:pc_autoencoding}. We use N=8 (a) and  resp. N=63 (b) blocks.}
\label{fig:architectures}
\end{figure*}

==> figs/qualitative_imgs/img_examples.tex <==
\begin{figure}[!t]
    \newcommand{\imgwidth}{0.1}
    \centering
    \begin{tabular}{ccc}
        Glow & Glow + LLM & Difference  \\
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/samples/2.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/samples_pp/2.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/diff/diff2.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/samples/3.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/samples_pp/3.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/diff/diff3.png} \\
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/samples/17.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/samples_pp/17.png} &
        \includegraphics[width=\imgwidth\textwidth]{figs/qualitative_imgs/diff/diff17.png} \\
    \end{tabular}
    \caption{Samples from Glow (+LLM) and the corresponding difference. The difference magnified such that its largest value is 255 for visualization purpose. The difference resembles white noise.}
    \label{fig:img_samples}
\end{figure}

==> figs/supplement_ablations/llm.tex <==
\begin{figure}[t!]
\centering
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figs/supplement_ablations/f1_vs_epochs.pdf}
  \caption{F1-Score depending on the number of epochs used for ManiFlow-LLM.}.
  \label{fig:f1_vs_epochs}
\end{subfigure}%
\\
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figs/supplement_ablations/f1_vs_dweight.pdf}
  \caption{F1-Score depending on the on the logarithm of the weight $\lambda$ used for ManiFlow-LLM.}
  \label{fig:f1_vs_dweight}
\end{subfigure}
\caption{Analysis of the sensitivity of ManiFlow-LLM to the number of epochs (a) and the magnitude of $\lambda$ (b) on the airplane category.}
\label{fig:llm_ablation}
\end{figure}

==> figs/supplement_ablations/llpoisson.tex <==
\begin{figure}
\centering
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figs/supplement_ablations/f1_vs_dpoisson.pdf}
  \caption{F1-Score depending on the depth used in Poisson surface reconstruction.}.
  \label{fig:f1_vs_dpoisson}
\end{subfigure}%
\\
\begin{subfigure}{.49\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figs/supplement_ablations/f1_vs_k1poisson.pdf}
  \caption{F1-Score depending on the on the logarithm of the number of points K\textsubscript{1}.}
  \label{fig:f1_vs_nr_points}
\end{subfigure}
\caption{Analysis of the sensitivity of ManiFlow-LL-Poisson to the depth used for Poisson surface reconstruction (a) and the number of points K\textsubscript{1} (b) on the airplane category.}
\label{fig:llpoisson_ablation}
\end{figure}

==> figs/toy_examples/regularization/vis.tex <==
\begin{figure*}[t!]
\begin{center}

    \renewcommand{\figsize}{0.16}
    
    \begin{tabular}{ c c c c c }
    
        \centering 
    
        GT & GT + Noise & NF & LLM, $\lambda=0.0$ & LLM, $\lambda=0.2$ \\
        
      \includegraphics[width=\figsize\linewidth]{figs/toy_examples/regularization/gt_no_noise.pdf} &
      \includegraphics[width=\figsize\linewidth]{figs/toy_examples/regularization/gt_small_noise.pdf} &
      \includegraphics[width=\figsize\linewidth]{figs/toy_examples/regularization/flow_noisy.pdf} &
      \includegraphics[width=\figsize\linewidth]{figs/toy_examples/regularization/flow_noisy_pp_no_reg.pdf} &
      \includegraphics[width=\figsize\linewidth]{figs/toy_examples/regularization/flow_noisy_pp_reg.pdf} \\
      
      
    \end{tabular}
    
\end{center}
\caption{In this experiment, we learn a non-uniform distribution (GT, GT + Noise) that exists on a 1D sine curve in 2D using a \ac{nf}. We demonstrate the importance of the regularization parameter $\lambda$. In absence of regularization ($\lambda =0$) LLM is not able to recover the correct distribution on the sine curve. However, using $\lambda = 0.2$ recovers the correct distribution.}\label{fig:toy_example_regularization}
\end{figure*}

==> tables/fid_images_uniform.tex <==
\begin{table}
\begin{center}
\caption{Quantitative evaluation on image generation. We report the FID score when training a GLOW model~\cite{kingma2018glow} on MNIST/CIFAR10/CelebA with and without post-processing. During training uniform noise is added to the images}
\label{table:headings}
\begin{tabular}{cccc}
\hline\noalign{\smallskip}
Post-processing & MNIST & CIFAR10 & CelebA\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
 \ding{55}  & 56.7              & 83.5            & 61.6            \\
 \ding{51}  & \textbf{50.8}     & \textbf{72.8}    & \textbf{50.9}    \\
\hline
\end{tabular}
\end{center}
\end{table}
